On the Error Resistance of Hinge Loss Minimization

Commonly used classification algorithms in machine learning, such as support vector machines, minimize a convex surrogate loss on training examples. In practice, these algorithms are surprisingly robust to errors in the training data. In this work, we identify a set of conditions on the data under which such surrogate loss minimization algorithms provably learn the correct classifier. This allows us to establish, in a unified framework, the robustness of these algorithms under various models on data as well as error. In particular, we show that if the data is linearly classifiable with a slightly non-trivial margin (i.e. a margin at least $C/\sqrt{d}$ for $d$-dimensional unit vectors), and the class-conditional distributions are near isotropic and logconcave, then surrogate loss minimization has negligible error on the uncorrupted data even when a constant fraction of examples are adversarially mislabeled.

==> files/missing_proofs.tex <==
\section{Missing Proofs from~\cref{sec:dense}}
\label{sec:missing_proofs}
\begin{proof}[Proof of Lemma~\labelcref{lem:i1term}]
Recall that $y\vz^\top \vv \leq 0$ and that $(\vx_i, y_i)$ is in $P_{\vv}^\tau(\vz, y)$ so that $y_i \vv^\top \vx_i \leq \tau$; by the assumption on $\tau$, this is at most $\gamma /2$. The fact that $\norm{\vw} \leq \frac 1 \gamma$ then implies the first claim.

% For a geometric proof of the second claim, see Figure~\ref{fig:pancakes}. An analytic proof follows.
Let $\vv^\top\vvstar = \alpha$. Note that
\begin{align*}
    y_i \vx_i^\top(\vvstar - (\vv^\top\vvstar)\vv) &\geq \gammastar - (\vv^\top\vvstar) \tau\\
    &= \gammastar - \alpha \tau,
\end{align*}
whereas
\begin{align*}
    \|\vvstar - (\vv^\top\vvstar)\vv\|^2 &= 1 + \alpha^2 - 2\alpha^2\\
    &= 1-\alpha^2.
\end{align*}
Thus
\begin{align*}
    y_i \vx_i^\top \vv' &\geq \frac{\gammastar - \alpha\tau}{\sqrt{1-\alpha^2}}.
\end{align*}
Setting the derivative with respect to $\alpha$ to zero, we can verify that this expression is minimized when $\alpha = \frac{\tau}{\gammastar}$. Plugging in this value immediately yields the result.
\end{proof}

% \begin{lem}\label{lem:oterm}
% For any set $O \subseteq \mcX \times \pmone$, and any $\vw$,
% \begin{align*}
%     \norm{\sum_{(\vx_i, y_i) \in O} \nabla_\vw\ell(\vw; \vx_i, y_i) }\leq L \cdot \linsumnorm(O).
% \end{align*}
% \end{lem}
\begin{proof}[Proof of Lemma~\labelcref{lem:oterm}]
Since $|f'(\cdot)| \leq L$, it follows that
\begin{align*}
\|\sum_{(\vx_i, y_i) \in O} \nabla_\vw\ell(\vw; \vx_i, y_i)\|
&= \|\sum_{(\vx_i, y_i) \in O} f'(y_i\vx_i^\top\vw) \cdot y_i \vx_i\|\\
&= L \cdot \|\sum_{(\vx_i, y_i) \in O}  \left(\frac{y_i f'(y_i\vx_i^\top\vw)}{L}\right)\cdot \vx_i \|\\
&\leq L \cdot\linsumnorm(O).
\end{align*}
\end{proof}

